Contrastive Conformal Sets

Contrastive learning produces coherent semantic feature embeddings by encouraging positive samples to cluster closely while separating negative samples. However, existing contrastive learning methods lack a principled construction of geometric sets in the semantic feature space with distribution-free guarantees at any user-specified coverage level. We extend conformal prediction to this setting by introducing covering sets equipped with learnable generalized hyper-ball constraints. We propose a method that constructs conformal sets guaranteeing user-specified coverage of positive samples while maximizing negative sample exclusion. We theoretically motivate volume minimization as a proxy for negative exclusion, enabling our approach to operate effectively even when negative pairs are unavailable. The positive inclusion guarantee inherits the distribution-free coverage property of conformal prediction, while negative exclusion is maximized through learned set geometry optimized on a held-out training split. Experiments on simulated and real-world image datasets demonstrate improved inclusion-exclusion trade-offs compared to standard distance-based conformal baselines.

==> latexmkrc <==
ensure_path( 'BIBINPUTS', './bib//' );
ensure_path( 'TEXINPUTS', './latex//' ); # E.g., path to directory containing your preamble.tex

##########################################
# #For use in Overleaf with xr package
##########################################

# $sub_doc_output = 'output-subdoc';

# # Options to supply to latexmk for compilation of external documents:
# @sub_doc_options = ('-cd', '-interaction=nonstopmode', '-file-line-error');

# push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# # Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

# push @file_not_found, '^No file\\s*(.+)\s*$';

# add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
# sub makeexternaldocument {
#     if ( $root_filename ne $_[0] )  {
#         my ($base_name, $path) = fileparse( $_[0] );
#         pushd $path;
#         my $return = system "latexmk",
#                             @sub_doc_options,
#                             "-aux-directory=$sub_doc_output",
#                             "-output-directory=$sub_doc_output",
#                             $base_name;
#         if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

#              rdb_add_generated( "$sub_doc_output/$base_name.aux" );
#              copy "$sub_doc_output/$base_name.aux", ".";
#         }
#         popd;
#         return $return;
#    }
# }

##########################################
##########################################

